Robot Action Selection Learning via Layered Dimension Informed Program Synthesis

Action selection policies (ASPs), used to compose low-level robot skills into complex high-level tasks are commonly represented as neural networks (NNs) in the state of the art. Such a paradigm, while very effective, suffers from a few key problems: 1) NNs are opaque to the user and hence not amenable to verification, 2) they require significant amounts of training data, and 3) they are hard to repair when the domain changes. We present two key insights about ASPs for robotics. First, ASPs need to reason about physically meaningful quantities derived from the state of the world, and second, there exists a layered structure for composing these policies. Leveraging these insights, we introduce layered dimension-informed program synthesis (LDIPS) - by reasoning about the physical dimensions of state variables, and dimensional constraints on operators, LDIPS directly synthesizes ASPs in a human-interpretable domain-specific language that is amenable to program repair. We present empirical results to demonstrate that LDIPS 1) can synthesize effective ASPs for robot soccer and autonomous driving domains, 2) requires two orders of magnitude fewer training examples than a comparable NN representation, and 3) can repair the synthesized ASPs with only a small number of corrections when transferring from simulation to real robots.

==> overview.tex <==

% \jh{Describe what happens UNSAT means one time here.}\\
% Stages of DIPS
\jb{Either here, or in the previous section, we need to make clear that LDIPS-L3 first generates the structure of an incomplete ASP by identifying all possible action transitions from the demonstrations, and then synthesizing a predicate blank for each possible transition. L2 is then invoked to fill in each predicate blank, and it in turn invokes L1 to fill in the parameter blanks.}
\technique{} consists of three stages that produce
complete action selection policies
given different levels of partially specified policies:\\
\begin{paraenum}
% L3 Description
\item At the highest layer, \technique{-L3} consumes
the set of demonstrations $\demos$
as a specification, and a type environment $\env$ that describes the
domain-specific
operations, $\const$, and $\inputVar$ that should be used for synthesis.
Each $\demo \in \demos$ is a tuple
$\demo = \langle$ start : $\action$, final : $\action$, in : $\world \rangle$,
and a $\world$ is a world state that maps
from $\inputVar$ to values,
$\world = [\inputVar^1 = \const_1,\dots,\inputVar^n = \const_n]$.
The goal
of \technique{-L3} is to find
a policy in the grammar that takes a current action $\startAction$ and a
world state $\world$
and outputs the next action. The policy, when
evaluated for each $\langle \demoStart, \demoIn \rangle \in \demos$
should produce $\demoFinal$.
Formally, we want to
find:
%
$p : \pol \mid \interp(p, \demoStart, \demoIn) =
  \demoFinal, \forall \demo \in \demos$

%\jh{May not be clear enough how L2 and L3 are different at this point}
% L2 Description
\item The second layer, \technique{-L2}, consumes a predicate sketch $\pred$
with expression holes $?\expr$ and parameter holes
$?\param$, the environment $\env$, and two sets of example world states,
and synthesizes a new predicate $\pred'$ that evaluates to
$\true$ on the positive examples $\posE = [\world]$,
and $\false$ on the negative examples $\negE = [\world]$.
$\posE$ and $\negE$ indicate whether a transition from a particular action
$\action_1$ to a subsequent action $\action_2$ should be
taken. Thus, $\posE$ and $\negE$ are subsets of $\world \in \demos$ that
start in $\action_1$.
$\pred'$ evaluated for all $\world \in \posE$
should result in $\true$, indicating that the robot should transition from $\action_1$
to $\action_2$, while $\pred'$ evaluated
for all $\world \in \negE$ should result in $\false$, indicating that the robot
should not transition.
Formally:
%
$\pred' : \pred \mid
  \interp(\pred', \world) = \textrm{\true}, \forall \world \in \posE \land
  \interp(\pred', \world) = \textrm{\false}, \forall \world \in \negE$

% L1 Description
\item The final layer, \technique{-L1},
consumes a sketch $\pred$ with parameter holes $?\param$,
and example sets $\posE, \negE$, and synthesizes a new predicate $\pred'$
by completing the sketch such that:\\
%
  $\pred' : \pred \mid
  \interp(\pred', \world) = \textrm{\true}, \forall \world \in \posE \land
  \interp(\pred', \world) = \textrm{\false}, \forall \world \in \negE$
\end{paraenum}

Each step of \technique{} builds on the lower layers to synthesize policies
with less user specification.
As such, in the following sections we will examine each layer of \technique{}
in detail from the bottom up, starting with \technique{-L1}.


==> problem.tex <==

Action selection learning is the task of learning a policy, that
given the current action and the state of the world
outputs the optimal next action to achieve some behavior.
When the goal behavior is described by a set of demonstrations
the goal of learning is to find a policy that is consistent with the
demonstrations, and that can generalize the behavior to unseen world states.
% $\demo \in \demos$, where
% $\demo = \langle \action_s, \action_f, \world \rangle$, the goal of learning
% is to find a policy
% %
% $p \mid p(\action_s, \world) =
  % \action_f, \forall \demo \in \demos$.
% %
In this work, we propose an approach to learning action selection from
demonstrations by guiding
learning with
a structured grammar for action selection and
Layered Dimension Informed Program Synthesis (\technique{}).


==> synthesis.tex <==
% Problem statement stuff
% The goal of this work is to utilize high-level user guidance, in the form
% of demonstrations, to synthesize action selection policies for composing disparate
% skills into a single behavior. Each skill is a distinct, self-contained feedback
% controller that is assumed to be \textit{convergent}, such that
% when certain preconditions are met, the controller will eventually
% achieve the desired result.

% Formally, given a set of robot controllers $\mathbf{C}$ and a set of world
% state variables $x{_y}{^i} \in \mathbf{W}$, we want to synthesize a
% function $T:\mathbf{W} \mapsto \mathbf{C}$ that maps
% $\mathbf{W}$ to $\mathbf{C}$ such that a behavior exemplified by some demonstrations
% is achieved.

% For this purpose, we model demonstrations as execution traces $\ptrace$ of the
% desired behavior. An execution trace is a sequence of \emph{trace elements}:
% \begin{align}
% \eqlabel{traceElement}
  % \trelt_t ::=  {\mktrelt
    % {\langle \limforall{i=1}{m} \pin{x^i} \pmapsto k^i \rangle}
    % { \mathbf{C}}}
% \end{align}
% that record the state $\mathbf{X}$ as the concrete values of $\pin{x^i}$,
% and the acting controller $s_t$ at time-step $t$. Each $\trelt_t$
% acts as an input/output (I/O) example for synthesis, and we
% will use a set of traces $\mathbf{R}$ to demonstrate the desired behavior.

We define a language for representing action
selection policies in terms of a grammar, shown in \figref{syntax},
where a policy $\pol$ is defined as a hierarchical set of predicates $\pbool$,
that output actions $\action$. Each $\bool$ in a $\pol$ is an arbitrary
sized composite conditional consisting of comparisons between
mathematical expressions $\expr$ and constant value threshold parameters \const.
Expressions $\expr$ are composed of unary operations \uOpE{}, and
binary operations \bOpE{} operating on program inputs \inputVar{}.
% Type Checking
This language supports real values $R$, vectors $V$,
and booleans as types (\type), and implements type checking.
The operations shown in \figref{syntax} demonstrate
the types of operations available to the language but are \emph{not} inclusive.
In particular, different domains require different sets of operations.

% Sketches
\technique{} employs \textit{sketches} to partially define and constrain the
structure of policies. A sketch is a partial program, where some
implementation details are left as \textit{holes} to be filled in
via synthesis \cite{combinatorialSketching}.
Sketches can be user-designed to guide \technique{}, or
generated at different stages of \technique{}
to represent partial solutions.
These sketches describe
the common structure of policies and can contain three types of holes,
predicate holes (?\bool) that are filled with conditional logic,
expression holes (?\expr) that are filled with mathematical operations,
and parameter holes (?\param) that are filled with real numbers.

% Syntax Figure
\begin{figure}[htb]
  \scriptsize
  \lstset{language=model}
  \begin{minipage}[t!]{0.27\textwidth}
    \(
    \begin{array}{@{}l@{}l@{}l@{\;}c@{\;}ll}
      %
      \multicolumn{6}{@{}l}{\textbf{Unary Operators}} \\
      \mathit{op}_1 & ::= &
      \multicolumn{4}{l}{\texttt{abs}
      \mid \texttt{sin}
      \mid \texttt{norm}
      \mid \cdots} \\[.4em]
      %
      \multicolumn{6}{@{}l}{\textbf{Binary Operators}} \\
      \mathit{op}_2 & ::= &
      \multicolumn{4}{l}{\texttt{+}
      \mid \texttt{-}
      \mid \texttt{*}
      \mid \texttt{dist}
      \mid \cdots} \\[.4em]
      %
      \multicolumn{6}{@{}l}{\textbf{Actions}} \\
      \action & ::= &
      \multicolumn{4}{l}{
        \mid \texttt{kick}
        % \mid \texttt{kick}
        \mid \texttt{cruise}
        \mid \cdots} \\[.4em]
      %
      \multicolumn{6}{@{}l}{\textbf{Constant Values}} \\
      \const & ::= &~\param & : &  \type &
      \hspace{0pt} \textrm{Parameter} \\
      & \mid & \realc & : & \type & \textrm{Real Value} \\
      & \mid & V & : & \type & \textrm{Real Valued Vector} \\
      & \mid & ?\param & : &T & \textrm{Parameter Hole} \\
      % \inputVar & ::= & \const:T &
      % \hspace{0pt} \textrm{Input Variable} \\ [.4em]
      %
      % \multicolumn{4}{@{}l}{\textbf{Sketch Holes}} \\
      % \hole{\bool} & ::= & \bool &
      % \hspace{0pt} \textrm{Predicate Hole} \\
      % \hole{\expr} & ::= & \expr & \hspace{0pt}
      % \textrm{Expression Hole} \\ \hole{\param} & ::= & \param &
      % \hspace{0pt} \textrm{Parameter Hole} \\ [.4em]
      % %
    \end{array}
    \)
    \(
    \begin{array}{@{}r@{\;}c@{\;}l@{\;}l}
      %
      \multicolumn{4}{@{}l}{\textbf{Types and Dimensions}} \\
      \dims & ::=  & \dimension{} & \textrm{Length, Time, Mass}  \\
            & \mid & [0, 0, 0] & \textrm{Dimensionless} \\
      \type & ::=  & \textrm{bool} & \textrm{Boolean}  \\
      & \mid & \dims
      & \textrm{Scalar with dimensions \dims} \\
      & \mid & \vect{(\dims)}
      & \textrm{2x1 matrix with dimensions \dims} \\[0.4em]
      %
    \end{array}
    \)
  \end{minipage}
  %
  \hspace{30pt}
  \vrule
  \hspace{5pt}
  %
  \begin{minipage}[t]{0.27\textwidth}
    \(
    \begin{array}{@{}r@{\;}c@{\;}l@{\;}l}
      %
      \multicolumn{4}{@{}l}{\textbf{Expressions}} \\
      \expr & ::=  & \inputVar:T & \textrm{Input Variable}\\
      & \mid & \multicolumn{2}{l}
      {\hspace{-6pt} \uOp{\expr}} \\
      & \mid & \multicolumn{2}{l}
      {\hspace{-6pt} \bOp{\expr_1}{\expr_2}} \\[.4em]
      & \mid & ?\expr & \textrm{Expression Hole} \\[.4em]
      %
      \multicolumn{4}{@{}l}{\textbf{Predicates}} \\
      \pbool & ::=  & \texttt{$\#t$~| $\#f$} \\
      & \mid & (\action_1~\texttt{==}~\action_2)
      & \hspace{0pt} \\
      & \mid & (\expr~\texttt{>}~\const) \\
      & \mid & (\expr~\texttt{<}~\const) \\
      & \mid & (\pbool_1~\&\&~\pbool_2) \\
      & \mid & (\pbool_1~||~\pbool_2) \\
      & \mid & ?\bool & \textrm{Predicate Hole} \\
      %
      \multicolumn{4}{@{}l}{\textbf{Action Selection Policy}} \\
      \pol & ::= & \texttt{return}~\action \\
      & \mid &
        \multicolumn{2}{@{}l}{\texttt{if (\bool) then $\pol_1$ else $\pol_2$}} \\
      %
    \end{array}
    \)
  \end{minipage}
  %
  % \hspace{1pt}
  \vrule
  \hspace{5pt}
  %
  \begin{minipage}[t!]{0.27\textwidth}
    %
    \(\begin{array}{@{}c@{\;}c@{\;}c@{}c@{}c@{}l@{\;}r}
      %
      \multicolumn{7}{@{}l}{\textbf{Types and Dimensions for Operations}} \\
      \uOpE & : & \multicolumn{3}{@{}c}{\type_1} & \rightarrow & \type_2  \\
      % \textrm{abs} & : & \type_1 & \rightarrow & \type_1  \\
      % + & : & \type_1 & \times & \type_1 & \rightarrow & \type_1  \\
      \textrm{abs} & : & \multicolumn{3}{@{}c}{\dims} &
          \rightarrow & \dims  \\
      \textrm{norm} & : & \multicolumn{3}{@{}c}{\vect(\dims)} &
          \rightarrow & \dims  \\
      \textrm{sin} & : & \multicolumn{3}{@{}c}{[0,0,0]} &
          \rightarrow & [0,0,0]  \\
      \bOpE & : & \type_1 & \times & \type_2 & \rightarrow & \type_3  \\
      + & : & \dims & \times & \dims &
          \rightarrow & \dims  \\
      % + & : & \multicolumn{3}{@{}c} {\dims  \times  \dims} &
          % \rightarrow & \dims  \\
      % + & : & \multicolumn{3}{@{}l} {\dims  \times  \dims} &
          % \rightarrow & \dims  \\
      + & : & \vect(\dims) & \times & \vect(\dims) &
          \rightarrow & \vect(\dims)  \\
      % * & : & \type_1 & \times & \type_1 & \rightarrow & \type_1  \\
      * & : & \dims_1 & \times & \dims_2 &
          \rightarrow & \dims_1 + \dims_2  \\
      * & : & \vect(\dims_1) & \times & \vect(\dims_2) &
          \rightarrow & \vect(\dims_1 + \dims_2)  \\
      / & : & \dims_1 & \times & \dims_2 &
          \rightarrow & \dims_1 - \dims_2  \\
      / & : & \vect(\dims_1) & \times & \vect(\dims_2) &
          \rightarrow & \vect(\dims_1 - \dims_2)  \\
      % % + & : & \vect[n_1, n_2, n_3] \times \vect[n_1, n_2, n_3] &
          % % \rightarrow & \vect[n_1, n_2, n_3]  \\
      % - & : & \type_1 \times \type_1 & \rightarrow & \type_1  \\
      % * & : & \type_1 \times \type_2 & \rightarrow & \type_1 + \type_2  \\
      % * & : & \type_1 \times \type_2 & \rightarrow & \type_1 + \type_2  \\
      %
    \end{array}\)
  \end{minipage}
  %
  \vspace{0.4em}
  \hrule
  \vspace{0.4em}
  %
  \caption{Grammar for action-selection policies.}
  \figlabel{syntax}
  % \vspace{-2em}
\end{figure}

\subsection{Dimensional Analysis}
% Why Dimensional Analysis
The program inputs for policies are measurable physical quantities drawn
from observations of the real world.
This offers a key characteristic that we can leverage to constrain the search
space: all mathematical operators must satisfy not
only type constraints but also dimensional analysis.
% What is dimensional analysis
Dimensional
analysis involves tracking base physical quantities
as calculations are performed, such that both the space of legal operations
is constrained, and the dimensionality of the result is well-defined. Quantities
can only be compared, added, or subtracted when they are commensurable, such
that they have the same dimensions, but they may be multiplied or divided even when
they are incommensurable.
% How do we implement all of this?
We extend the types \type of our language with dimensionality by defining
the dimension, ($\dims$), as the vector of dimensional
exponents $[n_1 * \mathit{Length}, n_2 * \mathit{Time}, n_3 * \mathit{Mass}]$.
Concretely,
if $\type$ represents length in meters then $\type=[1,0,0]$,
and if $\type$ represents a velocity vector such that
its dimensionality is $\mathit{Length / Time}$ then
$\type = \vect{([1,-1,0])}$.
Further, we extend the type signature of operations in our language to
include both dimensionality constraints that refine their domains, and
dimensionality effects that describe the result dimensions in terms of the
input dimensions.
% Examples in Figure
\figref{syntax} shows a representative
example of dimensional analysis and type rules for core
operators in our language.

% \begin{figure}
% \begin{center}
  % \setlength\tabcolsep{3pt} % default value: 6pt
  % \begin{tabular}{ c c l }
 % \hline
 % Operation & Constraint & Result Dim. \\
 % \hline
 % ($+$ $a$ $b$) & $Dim(a)$ $=$ $Dim(b)$ & $Dim(a)$ \\
 % ($-$ $a$ $b$) & $Dim(a)$ $=$ $Dim(b)$ & $Dim(a)$ \\
 % ($*$ $a$ $b$) & $-$ & $Dim(a) + Dim(b)$ \\
 % $(/~a~b)$ & $-$ & $Dim(a) - Dim(b)$ \\
 % $(\sin a)$ & $Dim(a) = [0,0,0]$  & $Dim(a)$ \\
 % \hline
% \end{tabular}
% \end{center}
% \caption{Examples of dimensional analysis for operators.}
% \figlabel{dimensions}
% \vspace{-0.5em}
% \end{figure}


==> technique.tex <==
% \begin{figure}[h]
  % \footnotesize
  % \begin{minipage}[htb!]{0.45\textwidth}

    % % technique
    % % \textrm{\technique{-L3}} : \nat * \env * \world * \set{\ops}
    % % \mapsto \pol

    % % \textrm{\technique{-L3}}(\depth, \env, \world, \set{\ops}) \uEqual

    % % Divide problem into a number of predicates
    % % For each Predicate hole DIPS-L3
    % % Create all possible sketches
    % % For each candidate from DIPS-L3 run DIPS-L2
    % %  Create all possible programs
    % % For each candidate from DIPS-L2 run DIPS-L1
    % % Create SMT formula and solve for each program
    % % \jh{Continue to fight this}

    % % \(\begin{array}{@{}c}

    % \begin{center}
      % \(\begin{array}{c}
        % \example \in \world \uEqual \set{<\state{s}, \state{o}, \set{\inputVar^i}>} \\
        % \sig(\expr, \world) \uEqual
        % \set{\expr(\world[0]), \expr(\world[0]), \dots \expr(\world[i])} \\
      % \end{array}\)
    % \end{center}
    % \begin{center}
      % \textbf{\technique{-L3}}
    % \end{center}
    % % \end{array}\)

    % \(\begin{array}{@{}l}
      % \textrm{\technique{-L3}}(\env, \world) \uEqual
      % \textrm{\technique{-L3}}(\env, \set{\world'}, \set{\sketch'}) \\
      % \quad \given \set{\world'},\set{\sketch'} \in \textrm{CreateSketches(\world)}
    % \end{array}\)

    % \(\begin{array}{@{}l}
      % \textrm{\technique{-L3}}(\env, \set{\world}, \set{\sketch}) \uEqual
      % \textrm{Unify(\technique{-L3}}(\env, \world', \sketch') \\
      % \quad \forall \ \world' \in \set{\world}, \sketch' \in \set{\sketch} \\
    % \end{array}\)

    % \(\begin{array}{@{}l}
      % \textrm{\technique{-L3}}(\env, \world, \sketch) \uEqual
      % \textrm{\technique{-L2}}(\depth, \env, \world', \sketch') \\
      % \quad \given \world', \sketch' \in \textrm{EnumPred}(\depth), \\
      % \qquad \textrm{\technique{-L2}}(\depth, \env, \world', \sketch')
      % \ != \textrm{UNSAT} \\
    % \end{array}\)

    % \(\begin{array}{@{}l}
      % \textrm{\jh{not handling the change of desired result to bool}}\\
      % \textrm{CreateSketches}(\world) \uEqual \set{\pair{\sketch'}{\world'}} \\
      % \given \sketch' \uEqual
      % \textrm{if}(\ \state{s}' \ \land \ ?\bool{}) \
      % \textrm{return } \state{o}', \\
      % \quad \state{s}' \uEqual \state{s} \in \world,
      % \state{o}' \uEqual \state{o} \in \world, \textrm{ and} \\
      % \quad \world' \uEqual \set{\example} \in \world \
      % \textrm{with} \ \state{s} == \state{s}' \\
      % \forall{} \ \state{s}',\state{o}' \in \world \\
    % \end{array}\)

    % %EnumPred
    % \(\begin{array}{@{}l@{}l@{\ }l@{\ }c@{\ }l}
      % % \multicolumn{5}{c}{ {\textrm{\textbf{PIP-L3}}} } \\
      % \multicolumn{5}{@{}l}{
        % \textrm{EnumPred}(\depth) \uEqual \set{\#t,\#f}} \\
      % \multicolumn{5}{@{}l}{
        % \textrm{EnumPred}(\depth{+1}) \uEqual} \\
      % \quad ?\expr \ > \ \ & ?\param & \land & c', &
      % \forall{} c' \in \textrm{EnumPred}(\depth) \ \cup \\
      % \quad ?\expr \ < \ \ & ?\param & \land & c', &
      % \forall{} c' \in \textrm{EnumPred}(\depth) \ \cup \\
      % \quad ?\expr \ > \ \ & ?\param & \lor & c', &
      % \forall{} c' \in \textrm{EnumPred}(\depth) \ \cup \\
      % \quad ?\expr \ < \ \ & ?\param & \lor & c', &
      % \forall{} c' \in \textrm{EnumPred}(\depth) \\
    % \end{array}
    % \)

    % \vspace{2pt}
    % \hrule
    % \vspace{2pt}

    % \begin{center}
      % \textbf{\technique{-L1}}
    % \end{center}

    % \(\begin{array}{@{}l}
      % \textrm{\technique{-L1}}(\world, \sketch, \set{\sig}) \uEqual \\
      % \quad \textrm{solve}(\exists \param, \ \forall \ ?\param \in \sketch',
      % \ \forall \example \in \world) \\
      % \quad \given \sketch' \uEqual \textrm{Peval}(\sketch, \example, \set{\sig})
    % \end{array}\)

  % \end{minipage}
  % \hfill
  % \vrule
  % \hfill
  % \begin{minipage}[t!]{0.45\textwidth}

    % \begin{center}
      % \textbf{\technique{-L2}}
    % \end{center}

    % \(\begin{array}{@{}l}
      % \textrm{\technique{-L2}}(\depth, \env, \world, \sketch) \uEqual
      % \textrm{\technique{-L1}}(\world, \sketch', \sig') \\
      % \quad \given \sketch',\sig' \in
      % \textrm{EnumFeature}(\depth, \env, \world, \type, ?\expr') \
      % \forall \ ?\expr' \ \in \sketch, \\
      % \qquad \textrm{\technique{-L1}}(\world, \sketch') \ != \textrm{UNSAT} \\
    % \end{array}\)

    % \(\begin{array}{@{}l@{}l@{}l}

      % % Type Signature / Definition
      % \multicolumn{3}{@{}l}{
        % \textrm{EnumFeature} : \nat * \env * \type * \world * \expr
        % \mapsto{}
        % \set{\fEnumOut{\expr}}
      % } \\

      % % Top Level Call
      % \textrm{EnumFeature}(\depth+1, \env, \type, \world, \eSym) & \uEqual{} \\
      % % Smaller Depth
      % \multicolumn{3}{@{}l}{ \quad
      % \textrm{EnumFeature}(\depth, \env, \type, \world, ?\expr{}) \ \cup
      % }\\
      % % Variables
      % \multicolumn{3}{@{}l}{ \quad
      % \textrm{EnumFeature}(\depth+1, \env, \type, \world, \inputVar),} \\
      % \multicolumn{3}{@{}l}{
        % \qquad{} \forall{} \inputVar : \type' \in \env
        % \given{} \type == \type' \in \env \ \cup
      % }\\
      % % uOp
      % \multicolumn{3}{@{}l}{ \quad
      % \textrm{EnumFeature}(\depth+1, \env, \type, \world, \uOpE'(?\expr),} \\
      % \multicolumn{3}{@{}l}{
        % \qquad{} \forall{} \uOpE' \in \uOpE
        % \given{}  \uOpE' : \type' \mapsto \type \in \env \ \cup}
      % \\
      % % bOp
      % \multicolumn{3}{@{}l}{ \quad
      % \textrm{EnumFeature}(\depth+1, \env, \type, \world, \bOpE'(?\expr, ?\expr)),} \\
      % \multicolumn{3}{@{}l}{ \qquad
      % \forall{} \bOpE' \in \bOpE
      % \given{} \bOpE' : \type' * \type'' \mapsto \type \in \env}\\
    % \end{array}
    % \)

    % % Variable Input
    % \(\begin{array}{@{}l@{}l@{}l}
      % &\textrm{EnumFeature}&(\depth, \env, \type, \world, \inputVar) \uEqual{} \\
      % & &\fEnumOut{\inputVar} \given{} \sig \uEqual{}
      % \set{\worldElem{1}{\inputVar},
      % \worldElem{2}{\inputVar}, \ldots{},
      % \worldElem{3}{\inputVar}} \\
    % \end{array}\)

    % % Operation1 Hole in Input
    % \(\begin{array}{@{}l@{}l@{}l}
      % &\textrm{EnumFeature}&(\depth{+1}, \env, \type, \world, \uOp{?\expr})
      % \uEqual
      % \set{\fEnumOut{\uOp{\expr'}}} \\
      % & &\forall{} \expr' \in
      % \textrm{EnumFeature}(\depth, \env, \type', \world, ?\expr), \\
      % & &\given \uOpE{} : \type' \mapsto{} \type \in \env, \\
      % & &\quad \sig \uEqual{} \map{\uOp{\expr'}}{\world} \\
    % \end{array}\)

    % % Operation2 Hole in Input
    % \(\begin{array}{@{}l@{}l@{}l}
      % &\textrm{EnumFeature}&(\depth{+1}, \env, \type, \world, \bOp{?\expr_1}{?\expr_2})
      % \uEqual \set{\fEnumOut{\bOp{\expr_1}{\expr_2}}} \\
      % & & \forall{} \expr_1 \in
      % \textrm{EnumFeature}(\depth, \env, \type', \world, ?\expr), \\
      % & & \forall{} \expr_2 \in
      % \textrm{EnumFeature}(\depth, \env, \type'', \world, ?\expr), \\
      % & & \given{} \bOpE : \type' * \type'' \mapsto{} \type \in \env, \\
      % & & \quad \sig \uEqual{} \map{\bOp{\expr_1}{\expr_2}}{\world} \\
    % \end{array}\)
  % \end{minipage}

  % \caption{\technique{} Synthesis}
  % \label{trace-compiler-figure}
% \end{figure}

\jh{Problem statement, inputs, outputs, overview of algorithm here!}

\subsection{\technique{-L1} : Parameter Synthesis}

\subsection{\technique{-L2} : Feature Synthesis}

\subsection{\technique{-L3} : Predicate Synthesis}

